Relativistic distortions in the large-scale clustering of SDSS-III BOSS CMASS galaxies

General relativistic effects have long been predicted to subtly influence the observed large-scale structure of the universe. The current generation of galaxy redshift surveys have reached a size where detection of such effects is becoming feasible. In this paper, we report the first detection of the redshift asymmetry from the cross-correlation function of two galaxy populations which is consistent with relativistic effects. The dataset is taken from the Sloan Digital Sky Survey DR12 CMASS galaxy sample, and we detect the asymmetry at the $2.7\sigma$ level by applying a shell-averaged estimator to the cross-correlation function. Our measurement dominates at scales around $10$ h$^{-1}$Mpc, larger than those over which the gravitational redshift profile has been recently measured in galaxy clusters, but smaller than scales for which linear perturbation theory is likely to be accurate. The detection significance varies by 0.5$\sigma$ with the details of our measurement and tests for systematic effects. We have also devised two null tests to check for various survey systematics and show that both results are consistent with the null hypothesis. We measure the dipole moment of the cross-correlation function, and from this the asymmetry is also detected, at the $2.8 \sigma$ level. The amplitude and scale-dependence of the clustering asymmetries are approximately consistent with the expectations of General Relativity and a biased galaxy population, within large uncertainties. We explore theoretical predictions using numerical simulations in a companion paper.

==> tex/simulation.tex <==
\section{Simulations}
Describe the Simulation used in the paper

==> tex/systematic.tex <==
\section{Systematic}
Largely refer to paper to but might need this section to talk about few specific things about the measurements procedure.
